A Bayesian semi-parametric model for longitudinal growth and appetite phenotypes in children

This study develops a Bayesian semi-parametric model to examine the longitudinal growth and appetite phenotypes in children from the GUSTO cohort, with a focus on understanding the relationship between eating behaviours and growth outcomes over time. While eating behaviours, such as picky eating, have been shown to influence future weight and obesity risk, their developmental patterns and associations with growth trajectories remain under-explored. This work addresses these gaps by modelling longitudinal data, including both growth metrics (e.g., BMI) and eating behaviours (e.g., Child Eating Behaviour Questionnaire, CEBQ), across multiple time points. We extend the Partial Credit Model, commonly used for questionnaire data analysis, to accommodate repeated measurements and incorporate covariates. The growth outcomes are modelled using flexible splines regression. The two components of the model are linked through a shared Bayesian nonparametric prior distribution, specifically a Normalized Generalized Gamma process, allowing to identify clinically relevant subgroups. This joint modelling approach offers a more nuanced understanding of how early eating behaviours relate to growth patterns and developmental outcomes, providing insights into childhood obesity risk.

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}
